Integrating Material Selection with Design Optimization via Neural Networks

The engineering design process often entails optimizing the underlying geometry while simultaneously selecting a suitable material. For a certain class of simple problems, the two are separable where, for example, one can first select an optimal material, and then optimize the geometry. However, in general, the two are not separable. Furthermore, the discrete nature of material selection is not compatible with gradient-based geometry optimization, making simultaneous optimization challenging. In this paper, we propose the use of variational autoencoders (VAE) for simultaneous optimization. First, a data-driven VAE is used to project the discrete material database onto a continuous and differentiable latent space. This is then coupled with a fully-connected neural network, embedded with a finite-element solver, to simultaneously optimize the material and geometry. The neural-network's built-in gradient optimizer and back-propagation are exploited during optimization. The proposed framework is demonstrated using trusses, where an optimal material needs to be chosen from a database, while simultaneously optimizing the cross-sectional areas of the truss members. Several numerical examples illustrate the efficacy of the proposed framework. The Python code used in these experiments is available at github.com/UW-ERSL/MaTruss

==> LiteratureReview.tex <==
\newpage
\section{Motivation}
\label{sec:motivation}
\subsection{Bullet points}
\begin{itemize}
    \item Talk about the design process involving geometric design, material selection, manufacturing process selection. interdependent phases
    \item Conventionally, these phases are carried out sequentially/independent of one another. drawbacks: longer development time, sub-optimal designs.
    \item This work considers the phases of structural design and material selection in conjunction.
    \item Talk about material selection - review ashby, and provide exampels of how ashby method is used in different application such as structural, thermal, other areas such as (while cost and structural perf are major features) biocompatibility, eco-friendly etc. inherently discrete
    \item geometric design ->  Talk about topology optimization conceptual design tool. TO for various design considerations such as fluid, thermal , struct. however, as noted in prev para, the mat selection also plays a pivotal role in dictating the perf. this necessitates that geom and mat selecting be done together.  inherently continuous. TO gradient descent. 
    \item Identify the problem in simultaneous optimization and material selection : The discrete nature of material selection space doesn't tie with the continuous nature of the geom design problem.
    \item Give references to works on above, and contibutions and drawbacks. Free material optimization.
    \item emphasize Differentiate between MMTO and the problem we are tackling.
    \item Contributions subsection.
    \begin{itemize}
        \item Pose the discrete material selection problem in a continuous space via NNs.
        \item highlight the challenges
    \end{itemize}
    talk a little bit about the methodology.
\end{itemize}
\subsection{Main}
    Engineering design is a sequence of decision making processes and activities which determine the form of an object to meet the target functional requirements \cite{eggert2005engineering}. The process of engineering design evolves over time in different design phases, first of which is the  `conceptual design' phase. Conceptual design is a phase in the engineering design process when alternative design concepts are synthesized, evaluated and selected for further development\cite{eggert2005engineering}. This phase is followed by the `embodiment design' phase \cite{dieter2009engineering}. The key design activities in this phase involves configuration of the structural layout (part geometry/topology), selecting the material and appropriate manufacturing processes \cite{dieter2009engineering}. \\
    Conventionally, the processes of geometry generation, material selection and manufacturing process selection are carried out sequentially and the alternative designs are analyzed to predict the performance. This is followed by redesign iteration in order to improve designs towards near-optimized configurations. This leads to an increased product development time, cost and possibly sub-optimized final designs. Structural designers ought to consider these processes simultaneously for optimized functional requirements \cite{rakshit2008simultaneous}. \textit{In this work, we intend to address this issue by considering the structural topology and material selection processes concurrently.}  
    
    
    
    
    
    
    
    \paragraph{Structural topology}{The structural design methods \textit{with assumed material} have been extensively studied under three categories: size, shape and topology optimization \cite{bendsoe2003topology}. Topology optimization (TO) has evolved as the preferred conceptual design tool for designing structures under multiple physics \cite{sigmund2001design}, multi-scale structures \cite{wu2021topology}, compliant mechanism design \cite{zhu2020design} and in the fields of architected material design \cite{osanov2016topology} to name a few. The approaches for topology optimization include the While there have been a variety of TO approaches \cite{sigmund2013topology}, most of the methods adopt gradient-based methods and continuous design variables to solve the constrained optimization problem \cite{sigmund2011usefulness}.
    }
    
    \paragraph{Material Selection}{The selection of material  \textit{with assumed geometry} is a well studied field. Refer to \cite{jahan2010material} for a comprehensive review of material choosing methods. Of the methods, Ashby's Method \cite{Ashby1993MaterialSelection} remains one of the most popular. Ashby's method primarily uses the material charts and performance indices to determine the best material from a database under the target requirements. This method is popular because of it's simplicity, efficiency and reliability, and has been used for selecting materials for aerospace systems \cite{arnold2012materials}, MEMS \cite{parate2011material}, nuclear applications \cite{hosemann2018materials}. Ashby Charts have also considered parameters beyond physical properties, such as manufacturing processes and costs, eco-friendliness, sustainability etc. \cite{ashby2013materials}. Unlike the TO problem, material selection from a database is inherently a discrete problem, and developing the performance indices for certain discrete parameters is not trivial.}
    
    
    
    \paragraph{Problem identification}{The challenge in integrating topology optimization and material selection is that the TO problem is inherently continuous, whereas the material selection problem is discrete. This makes it unsuitable for use in the gradient-based optimization schemes. }
    
    
    \paragraph{Previous works}{While there have been strides in both the domains (of topology optimization with assumed material and  material selection with assumed geometry) there has been little literature that simultaneously handles structural design and material selection. Ananthasuresh and Ashby \cite{ananthasuresh2003concurrent} made the first attempt to concurrently design a 3-bar truss system and select the single best material, using a design-index inspired from Ashby's charts. This was extended to the design of determinate truss systems \cite{rakshit2008simultaneous}, and further for the design of compliant mechanisms \cite{hegde2010design}. \cite{achleitner2022material} \cite{andersen2021competition}} Discuss about the design index by Anathsuresh.
    
    
    \paragraph{Differences between MMTO}{We emphasise that the proposed integration of topology optimization and material selection is fundamentally different from the works in the multi-material topology optimization area \cite{zuo2017multi},\cite{zhang2018multi}, \cite{Mirzendehdel2015MMTO}. In MMTO, the candidate materials are selected/chosen before-hand, and the domain is populated with one or more of these candidate material choices under certain constraints. In the present work, we seek to select the best material directly from a database of materials in conjunction to solving the topology optimization problem.}
    
    \paragraph{Contributions}
    
    Two key contributions in this paper
    
    \begin{enumerate}
        \item We encode the discrete material data into a continuous, differentiable space. We achieve this using a data-driven variational autoencoders.  We highlight the human interpretability of the encoded domain.
        \item We utilize the encoded, differentiable material space to simultaneously optimize the topology and corresponding choice of material via a physics-driven optimizaiton of neural networks. We showcase the optimization of structural and thermal designs under cost/mass and volume constraints. The topologies may be allocated with one or more materials.
    \end{enumerate}
    
    Other salient contributions are:
    



\newpage




==> preamble.tex <==

\usepackage{arxiv}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}
\usepackage{graphicx}

\usepackage{amsmath}
\usepackage{bm}

\usepackage{txfonts}
%\usepackage{natbib}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}

\usepackage{graphicx}
\usepackage{natbib}
\usepackage{doi}
\usepackage{authblk}
\usepackage{mathtools}
\usepackage{todonotes}
\usepackage{tablefootnote}
\usepackage{tabu}
\makeatletter
%\def\cl@chapter{\cl@chapter \@elt {theorem}}%bug in class
\def\cl@chapter{\@elt {theorem}}
\makeatother
\usepackage{cleveref}
\usepackage{dblfloatfix} 
\usepackage{tikz}
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
% My own commands
\newcommand*{\affaddr}[1]{#1} % No op here. Customize it for different styles.
\newcommand*{\affmark}[1][*]{\textsuperscript{#1}}
%\newcommand*{\email}[1]{\texttt{#1}}

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
